Surface-dominated conductance scaling in Weyl semimetal NbAs

Protected surface states arising from non-trivial bandstructure topology in semimetals can potentially enable new device functionalities in compute, memory, interconnect, sensing, and communication. This necessitates a fundamental understanding of surface-state transport in nanoscale topological semimetals. Here, we investigate quantum transport in a prototypical topological semimetal NbAs to evaluate the potential of this class of materials for beyond-Cu interconnects in highly-scaled integrated circuits. Using density functional theory (DFT) coupled with non-equilibrium Green's function (NEGF) calculations, we show that the resistance-area RA product in NbAs films decreases with decreasing thickness at the nanometer scale, in contrast to a nearly constant RA product in ideal Cu films. This anomalous scaling originates from the disproportionately large number of surface conduction states which dominate the ballistic conductance by up to 70% in NbAs thin films. We also show that this favorable RA scaling persists even in the presence of surface defects, in contrast to RA sharply increasing with reducing thickness for films of conventional metals, such as Cu, in the presence of surface defects. These results underscore the promise of topological semimetals like NbAs as future back-end-of-line (BEOL) interconnect metals.

==> Makefile <==
all: main
PDFLATEX=pdflatex --halt-on-error

main: main.tex
	$(PDFLATEX) main.tex
	bibtex main
	$(PDFLATEX) main.tex
	$(PDFLATEX) main.tex

SI: SI.tex
	$(PDFLATEX) SI.tex
	bibtex SI
	$(PDFLATEX) SI.tex

CoverLetter: CoverLetter.tex
	$(PDFLATEX) CoverLetter.tex
	$(PDFLATEX) CoverLetter.tex

Response1: Response1.tex
	$(PDFLATEX) Response1.tex
	$(PDFLATEX) Response1.tex

Response2: Response2.tex
	$(PDFLATEX) Response2.tex
	$(PDFLATEX) Response2.tex

submit: main
	awk '{ if($$1=="\\bibliography{ref}") print "\\input{main.bbl}"; else print; }' main.tex > temp.tex
	latexpand temp.tex > submit/submit.tex
	rm temp.tex


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
